Protein Representation Learning by Capturing Protein Sequence-Structure-Function Relationship

The goal of protein representation learning is to extract knowledge from protein databases that can be applied to various protein-related downstream tasks. Although protein sequence, structure, and function are the three key modalities for a comprehensive understanding of proteins, existing methods for protein representation learning have utilized only one or two of these modalities due to the difficulty of capturing the asymmetric interrelationships between them. To account for this asymmetry, we introduce our novel asymmetric multi-modal masked autoencoder (AMMA). AMMA adopts (1) a unified multi-modal encoder to integrate all three modalities into a unified representation space and (2) asymmetric decoders to ensure that sequence latent features reflect structural and functional information. The experiments demonstrate that the proposed AMMA is highly effective in learning protein representations that exhibit well-aligned inter-modal relationships, which in turn makes it effective for various downstream protein-related tasks.

==> 2_related_work.tex <==
\section{Related Work}
Previous uni-modal sequence- or structure-based methods can capture properties of proteins thanks to the vast amount of protein data available, they are limited to learning a single modality of proteins and cannot obtain comprehensive protein representations.
On the other hand, previous contrastive learning-base multi-modal protein representation learning may not be an optimal choice for multi-modal protein representation learning, as it essentially focuses on learning improved representations of a single modality using other modal information and thus cannot yield balanced multi-modal representations.
To overcome the limitations of previous works, our proposed AMMA first leverages a unified multi-modal encoder to integrate information from three different protein modalities to obtain a balanced multi-modal representation. AMMA further utilizes asymmetric decoders designed to accommodate the asymmetric sequence-structure-function relationship of proteins. Together, these make AMMA an effective multi-modal protein representation learning method for obtaining comprehensive protein representations.
Detailed previous works can be found in Section~\ref{sec:related_works}.


% \subsection{Uni-modal Protein Representation Learning}
% For learning protein representations using a single modality, the most basic and widely used is the sequence of the protein, i.e., a linear chain of amino acid residues. Many previous sequence-based protein representation learning methods have utilized language modeling techniques such as masked language modeling (MLM)~\citep{devlin2018bert}. ProtBERT~\citep{elnaggar2021prottrans} used BERT~\citep{devlin2018bert} to reconstruct missing amino acid residues. ESM-1b~\citep{rives2021biological} conducted masked language modeling (MLM) unsupervised learning on 250M protein sequences. ESM-1v~\citep{meier2021language} focused on capturing the effect of variations in sequence on function. ESM-2~\citep{lin2022language} proposed a language model with the larger 15B parameters than ESM-1b. \citet{heinzinger2022contrastive} proposed to obtain optimized sequence embeddings for the CATH protein structure hierarchy~\citep{orengo1997cath} by using contrastive learning to maximize the distance between sequences from different CATH classes and minimize the distance for those within the same class. Recently, the importance of structural information in learning protein representations has came to the fore and recent works have been proposed to exploit structural features in protein 3D geometry. \citet{hermosilla2022contrastive} and \citet{zhang2022protein} proposed to learn geometric features through contrastive learning between substructures of a given protein.
% % While these sequence- or structure-based methods can capture properties of proteins thanks to the vast amount of protein data available, they are limited to learning a single modality of proteins and cannot obtain comprehensive protein representations.

% \vspace{-0.05in}
% \subsection{Multi-modal Protein Representation Learning}
% \vspace{-0.05in}
% \paragraph{Contrastive Learning-based Multi-modal Learning}
% As a means to overcome the limitations of uni-modal protein representation learning, protein representation learning using multiple modalities has gained traction. Most previous studies have adopted a contrastive learning approach to capture the relationship between modalities. \citet{zhang2022ontoprotein} employed knowledge-aware negative sampling to identify negative instances, enabling contrastive learning across proteins. \citet{xu2023protst} conducted contrastive learning between protein sequence and functional description. \citet{zhang2024pepharmony} utilized ESM~\citep{rives2021biological} and GearNet~\citep{zhang2022protein} to encode sequence and structure data, respectively, and performed contrastive learning between the encoded sequence and structure features. %However, contrastive learning may not be an optimal choice for multi-modal protein representation learning, as it essentially focuses on learning improved representations of a single modality using other modal information and thus cannot yield balanced multi-modal representations.

% \vspace{-0.15in}
% \paragraph{Other Multi-modal Learning Approaches}
% Apart from contrastive learning, there are other approaches to multi-modal protein representation learning. \citet{chen2023structure} incorporated protein structural information by learning to predict residue distance or dihedral angle. This work also proposed to maximize the mutual information between the sequential representation and structural representation. \citet{su2023saprot} proposed using structure-aware tokens extracted from FoldSeek~\citep{van2022foldseek} to train a token-based ESM~\citep{lin2022language} backbone. These methods showed superior results as they consider the structure of proteins. However, the method of \citet{chen2023structure} has the limitation that it only uses sequence information as an auxiliary to guide and enhance structural representation. The method of \citet{su2023saprot} uses 20 different structural tokens, which restricts diversity when encoding structural information. Moreover, these methods do not consider another important modality for proteins, the function description, and are therefore suboptimal.

% To overcome all of the above limitations, our proposed AMMA first leverages a unified multi-modal encoder to integrate information from three different protein modalities to obtain a balanced multi-modal representation. AMMA further utilizes asymmetric decoders designed to accommodate the asymmetric sequence-structure-function relationship of proteins. Together, these make AMMA an effective multi-modal protein representation learning method for obtaining comprehensive protein representations.


==> figures/masking.tex <==
\begin{figure}[htbp]
    \centering
    \includegraphics[width=\columnwidth]{figures_pdf/masking.pdf}
    \caption{\textbf{Masking Strategy.}}
    \label{fig:masking}
\end{figure}

